Non-reversible Parallel Tempering for Deep Posterior Approximation

Parallel tempering (PT), also known as replica exchange, is the go-to workhorse for simulations of multi-modal distributions. The key to the success of PT is to adopt efficient swap schemes. The popular deterministic even-odd (DEO) scheme exploits the non-reversibility property and has successfully reduced the communication cost from $O(P^2)$ to $O(P)$ given sufficiently many $P$ chains. However, such an innovation largely disappears in big data due to the limited chains and few bias-corrected swaps. To handle this issue, we generalize the DEO scheme to promote non-reversibility and propose a few solutions to tackle the underlying bias caused by the geometric stopping time. Notably, in big data scenarios, we obtain an appealing communication cost $O(P\log P)$ based on the optimal window size. In addition, we also adopt stochastic gradient descent (SGD) with large and constant learning rates as exploration kernels. Such a user-friendly nature enables us to conduct approximation tasks for complex posteriors without much tuning costs.

==> AAAI_2023_Non-reversible_Parallel_Tempering - Clearn_version_for_arXiv (1)/chapters/checklist.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section*{Checklist}


% %%% BEGIN INSTRUCTIONS %%%
% The checklist follows the references.  Please
% read the checklist guidelines carefully for information on how to answer these
% questions.  For each question, change the default \answerTODO{} to \answerYes{},
% \answerNo{}, or \answerNA{}.  You are strongly encouraged to include a {\bf
% justification to your answer}, either by referencing the appropriate section of
% your paper or providing a brief inline description.  For example:
% \begin{itemize}
%   \item Did you include the license to the code and datasets? \answerYes{See Section~\ref{gen_inst}.}
%   \item Did you include the license to the code and datasets? \answerNo{The code and the data are proprietary.}
%   \item Did you include the license to the code and datasets? \answerNA{}
% \end{itemize}
% Please do not modify the questions and only use the provided macros for your
% answers.  Note that the Checklist section does not count towards the page
% limit.  In your paper, please delete this instructions block and only keep the
% Checklist section heading above along with the questions/answers below.
% %%% END INSTRUCTIONS %%%


\begin{enumerate}


\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{}
  \item Did you describe the limitations of your work?
    \answerYes{}
  \item Did you discuss any potential negative societal impacts of your work?
    \answerNA{}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{}
\end{enumerate}


\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerYes{}
        \item Did you include complete proofs of all theoretical results?
    \answerYes{}
\end{enumerate}


\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerYes{}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerYes{}
        \item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerYes{}
        \item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerNo{}
\end{enumerate}


\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
   \answerYes{}
  \item Did you mention the license of the assets?
   \answerNA{}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerNA{}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
     \answerNA{}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
     \answerNA{}
\end{enumerate}


\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerNA{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
   \answerNA{}
\end{enumerate}


\end{enumerate}

==> AAAI_2023_Non-reversible_Parallel_Tempering - Clearn_version_for_arXiv (1)/chapters/conclusion.tex <==

\section{Conclusion}


In this paper, we show how to adapt the multiple-chain parallel tempering algorithm to big data problems. Given a limited budget of parallel chains in big data, we show the standard non-reversible DEO scheme leads to an expensive quadratic communication cost with respect to the number of chains. To tackle that issue, we propose a generalized DEO scheme to achieve larger swap rates (window-wise) with mild costs. By sacrificing a mild accuracy in big data, we prove the existence of an optimal window size to encourage \emph{deterministic paths} and obtain in a significant \emph{acceleration of $O(\frac{P}{\log P})$ times}. For a user-friendly purpose, we also propose a deterministic swap condition to interact with SGD-based exploration kernels. A crude bias analysis is provided to facilitate the understanding of the extensions.

\section{Acknowledgments}

Lin and Deng would like to acknowledge the support from National Science Foundation (DMS-2053746, DMS-1555072, and DMS-1736364), Brookhaven National Laboratory Subcontract (382247), and U.S. Department of Energy Ofﬁce of Science Advanced Scientiﬁc Comput-ing Research (DE-SC0021142). Liang’s research is supported in part by the grant DMS-2015498 from National Science Foundation and the grants R01-GM117597 and R01-GM126089 from National Institutes of Health. 
% how to conduct efficient PT in big data problems. 


% To tackle the inefficiency issue of the popular DEO scheme given limited chains, 



% we present the DEO$_{\star}$ scheme by applying an optimal window size to encourage \emph{deterministic paths} and obtain in a significant \emph{acceleration of $O(\frac{P}{\log P})$ times}. For a user-friendly purpose, we propose a deterministic swap condition to interact with SGD-based exploration kernels and provide a theoretical guarantee to control the bias solely depending on the learning rate $\bm{\eta}$ and the correction buffer $\mathbb{C}$; we also provide a practical algorithm to adaptively approximate $\bm{\eta}$ and $\mathbb{C}$ for achieving the optimal efficiency in \emph{constrained settings}.

==> AAAI_2023_Non-reversible_Parallel_Tempering - Clearn_version_for_arXiv (1)/chapters/experiments.tex <==

\section{Experiments}
% \vskip -0.05in
\subsection{Simulations of multi-modal distributions}



We first simulate the proposed algorithm on a distribution $\pi(\bbeta)\propto \exp(-U(\bbeta))$, where $\bbeta=(\beta_1, \beta_2)$, $U(\bbeta)=0.2(\beta_1^2+\beta_2^2)-2(\cos(2\pi \beta_1)+\cos(2\pi \beta_2))$. The heat map is shown in Figure \ref{truth_density} with 25 modes of different volumes. To mimic big data scenarios, we can only access stochastic gradient $\nabla\widetilde U(\bbeta)=\nabla U(\bbeta)+2\mathcal{N}(0, \bm{I}_{2\times2})$ and stochastic energy $\widetilde U(\bbeta)=U(\bbeta)+2\mathcal{N}(0, I)$. 


% NIPS submission 
% \begin{figure*}[!ht]
%   \centering
%   \vskip -0.05in
%   \subfigure[\scriptsize{Ground truth} ]{\label{truth_density}\includegraphics[width=1.9cm, height=1.9cm]{figures/ground_truth_NRPT_iters_20000_chains_16_lr_0.01_0.5_sz_100_swap_rate_0.4_scale_2_window_8_seed_8.png}}\qquad
%   \subfigure[$\mathbb{S}=0.2$]{\includegraphics[width=1.9cm, height=1.9cm]{figures/NRPT_density_iters_20000_chains_16_lr_0.01_0.5_sz_100_swap_rate_0.2_scale_2_window_16_seed_12343.png}}\quad
%   \subfigure[$\mathbb{S}=0.3$]{\includegraphics[width=1.9cm, height=1.9cm]{figures/NRPT_density_iters_20000_chains_16_lr_0.01_0.5_sz_100_swap_rate_0.3_scale_2_window_10_seed_12343.png}}\quad
%   \subfigure[$\mathbb{S}=0.4$]{\includegraphics[width=1.9cm, height=1.9cm]{figures/NRPT_density_iters_20000_chains_16_lr_0.01_0.5_sz_100_swap_rate_0.4_scale_2_window_8_seed_666.png}}\quad
%   \subfigure[$\mathbb{S}=0.5$]{\includegraphics[width=1.9cm, height=1.9cm]{figures/NRPT_density_iters_20000_chains_16_lr_0.01_0.5_sz_100_swap_rate_0.5_scale_2_window_5_seed_12343.png}}\quad
%   \subfigure[$\mathbb{S}=0.6$]{\includegraphics[width=1.9cm, height=1.9cm]{figures/NRPT_density_iters_20000_chains_16_lr_0.01_0.5_sz_100_swap_rate_0.6_scale_2_window_4_seed_12343.png}}
%     \vskip -0.05in
%   \caption{\footnotesize{Study of different target swap rate $\mathbb{S}$ via DEO$_{\star}$-SGD, where SGLD is the exploitation kernel.}}
%   \label{test_of_acceptance_rates}
%   \vspace{-0.4em}
% \end{figure*}



% AAAI submission
\begin{figure}[!ht]
  \centering
  \vskip -0.05in
  \subfigure[\scriptsize{Truth} ]{\label{truth_density}\includegraphics[width=1.7cm, height=1.7cm]{figures/ground_truth_NRPT_iters_20000_chains_16_lr_0.01_0.5_sz_100_swap_rate_0.4_scale_2_window_8_seed_8.png}}\ \ 
  \subfigure[$\mathbb{S}=0.2$]{\includegraphics[width=1.7cm, height=1.7cm]{figures/NRPT_density_iters_20000_chains_16_lr_0.01_0.5_sz_100_swap_rate_0.2_scale_2_window_16_seed_12343.png}} \ \ 
%   \subfigure[$\mathbb{S}=0.3$]{\includegraphics[width=1.9cm, height=1.9cm]{figures/NRPT_density_iters_20000_chains_16_lr_0.01_0.5_sz_100_swap_rate_0.3_scale_2_window_10_seed_12343.png}}\quad
  \subfigure[$\mathbb{S}=0.4$]{\includegraphics[width=1.7cm, height=1.7cm]{figures/NRPT_density_iters_20000_chains_16_lr_0.01_0.5_sz_100_swap_rate_0.4_scale_2_window_8_seed_666.png}} \ \ 
%   \subfigure[$\mathbb{S}=0.5$]{\includegraphics[width=1.9cm, height=1.9cm]{figures/NRPT_density_iters_20000_chains_16_lr_0.01_0.5_sz_100_swap_rate_0.5_scale_2_window_5_seed_12343.png}}\quad
  \subfigure[$\mathbb{S}=0.6$]{\includegraphics[width=1.7cm, height=1.7cm]{figures/NRPT_density_iters_20000_chains_16_lr_0.01_0.5_sz_100_swap_rate_0.6_scale_2_window_4_seed_12343.png}}
    \vskip -0.05in
  \caption{\footnotesize{Study of different target swap rate $\mathbb{S}$ via DEO$_{\star}$-SGD, where SGLD is the exploitation kernel.}}
  \label{test_of_acceptance_rates}
  \vspace{-0.4em}
\end{figure}

We first run DEO$_{\star}$-SGD$\times$P16 based on 16 chains and 20,000 iterations. We fix the lowest learning rate 0.003 and the highest learning 0.6 and propose to tune the target swap rate $\mathbb{S}$ for the acceleration-accuracy trade-off. Figure \ref{test_of_acceptance_rates} shows that fixing $\mathbb{S}=0.2$ %or 0.3 
is too conservative and underestimates the uncertainty on the corners; $\mathbb{S}=0.6$ results in too many radical swaps and eventually leads to crude estimations; by contrast, $\mathbb{S}=0.4$ yields the best posterior approximation among the five choices. 



\begin{table*}[ht]
\begin{sc}
\vspace{-0.05in}
% \footnotesize
\caption[Table caption text]{posterior approximation and optimization on CIFAR100 via $10\times$ budget.} \label{UQ_test}
\vspace{-0.05in}
\begin{center} 
\begin{tabular}{c|cc|cc|cc}
\hline
\multirow{2}{*}{Model} & \multicolumn{2}{c|}{R\upshape{es}N\upshape{et}20} & \multicolumn{2}{c|}{R\upshape{es}N\upshape{et}32} & \multicolumn{2}{c}{R\upshape{es}N\upshape{et}56}  \\
\cline{2-7}
 &  NLL  & ACC (\%) & NLL & ACC (\%) & NLL  & ACC (\%) \\
\hline
\hline
{\upshape{cyc}SGHMC$\times$T10} &  8198$\pm$59 & 76.26$\pm$0.18  &  7401$\pm$28 & 78.54$\pm$0.15 & 6460$\pm$21 & 81.78$\pm$0.08  \\ 
{\upshape{cyc}SWAG$\times$T10} &   8164$\pm$38 & 76.13$\pm$0.21  & 7389$\pm$32 & 78.62$\pm$0.13 & 6486$\pm$29 & 81.60$\pm$0.14 \\ 
\hline
\hline
{\upshape{m}SGD$\times$P10} &  7902$\pm$64 & 76.59$\pm$0.11 & 7204$\pm$29 & 79.02$\pm$0.09  & 6553$\pm$15  & 81.49$\pm$0.09    \\ 
{DEO-\upshape{m}SGD$\times$P10} &  7964$\pm$23  & 76.84$\pm$0.12  & 7152$\pm$41 & 79.34$\pm$0.15 & 6534$\pm$26 & 81.72$\pm$0.12 \\ 
{$\text{DEO}_{\star}$-\upshape{m}SGD$\times$P10} &  \textbf{7741$\pm$67} & \textbf{77.37$\pm$0.16} & \textbf{7019$\pm$35} & \textbf{79.54$\pm$0.12} & \textbf{6439$\pm$32} & \textbf{82.02$\pm$0.15} \\ 
\hline
\end{tabular}
\end{center}
\end{sc}
\vspace{-0.05in}
\end{table*}

\begin{figure}[!ht]
  \centering
  \vskip -0.05in
  \subfigure[Round trips]{\label{round_trip_simulation}\includegraphics[width=2.5cm, height=2.5cm]{figures/optimal_window_size_NRPT_iters_20000_chains_16_lr_0.003_0.6_sz_100_swap_rate_0.4_scale_2_window_8_seed_888.png}}
  \subfigure[Learning rates]{\includegraphics[width=2.5cm, height=2.5cm]{figures/learning_rate_NRPT_iters_20000_chains_16_lr_0.003_0.6_sz_100_swap_rate_0.4_scale_2_window_8_seed_888.png}} 
  \subfigure[{Accept rates}]{\includegraphics[width=2.5cm, height=2.5cm]{figures/acceptance_iters_2000_chains_16_lr_0.01_0.5_sz_100_swap_rate_0.4_scale_2_window_8_seed_8.png}}
%   \subfigure[Corrections]{\label{correction_simulations}\includegraphics[width=2.5cm, height=2.5cm]{figures/correction_NRPT_iters_20000_chains_16_lr_0.003_0.6_sz_100_swap_rate_0.4_scale_2_window_8_seed_888.png}}\quad
    \vskip -0.05in
  \caption{Study of window sizes, learning rates, acceptance rates, and the corrections.}
  \label{learning_rate_acceptance_rate}
  \vspace{-0.5em}
\end{figure}

Next, we select $\mathbb{S}=0.4$ and study the round trips. We observe in Figure \ref{round_trip_simulation} that the vanilla DEO only yields 18 round trips every 1,000 iterations; by contrast, slightly increasing $W$ tends to improve the efficiency significantly and the optimal 45 round trips are achieved at $W=8$, which \emph{matches our theory}. In Figure \ref{learning_rate_acceptance_rate}(b-c), the geometrically initialized learning rates lead to unbalanced acceptance rates in the early phase and some adjacent chains have few swaps and others swap too much, but as the optimization proceeds, the learning rates gradually converge. %We also observe in Figure \ref{correction_simulations} that the correction is adaptively estimated to ensure the average acceptance rates converge to $\mathbb{S}=0.4$.

\begin{figure}[!ht]
  \centering
  % \vskip -0.07in
  \subfigure[{Truth} ]{\label{multi_density_truth}\includegraphics[width=1.4cm, height=1.4cm]{figures/ground_truth_NRPT_iters_20000_chains_16_lr_0.01_0.5_sz_100_swap_rate_0.4_scale_2_window_8_seed_8.png}}
  \subfigure[\footnotesize{SGLD}]{\label{sgld_parallel}\includegraphics[width=1.4cm, height=1.4cm]{figures/NRPT_density_sgld_ensemble_iters_20000_chains_16_lr_0.003_0.6_sz_100_swap_rate_0.4_scale_2_window_8_seed_888.png}}
  \subfigure[\tiny{cycSGLD}]{\label{cycSGLD_parallel}\includegraphics[width=1.4cm, height=1.4cm]{figures/NRPT_density_cyclic_sgld_iters_20000_chains_16_lr_0.003_0.6_sz_100_swap_rate_0.4_scale_2_window_8_seed_888.png}}
  \subfigure[\tiny{$\text{DEO}$-SGD}]{\label{DEO_parallel}\includegraphics[width=1.4cm, height=1.4cm]{figures/NRPT_density_NRPT_iters_20000_chains_16_lr_0.01_0.5_sz_100_swap_rate_0.4_scale_2_window_1_seed_8.png}}
  \subfigure[\tiny{$\text{DEO}_{\star}$-SGD}]{\label{deo_star_parallel}\includegraphics[width=1.7cm, height=1.6cm]{figures/NRPT_density_NRPT_iters_20000_chains_16_lr_0.01_0.5_sz_100_swap_rate_0.4_scale_2_window_8_seed_8.png}}
    % \vskip -0.05in
  \caption{Simulations of the multi-modal distribution through different sampling algorithms. All the algorithms are run based on 16 chains $\times P16$}
  \label{multi_modal_simulation}
  % \vspace{-0.5em}
\end{figure}


We compare the proposed algorithm with parallel SGLD based on 20,000 iterations and 16 chains (SGLD$\times$P16); we fix the learning rate 0.003 and a temperature 1. We also run cycSGLD$\times$T16, which denotes a single chain based on 16 times of budget and cosine learning rates \citep{ruqi2020} of 100 cycles. We see in Figure \ref{sgld_parallel} that SGLD$\times$P16 has good explorations but fails to approximate the posterior. Figure \ref{cycSGLD_parallel} shows that cycSGLD$\times$T16 explores most of the modes but overestimates some areas occasionally. Figure \ref{DEO_parallel} demonstrates the DEO-SGD with 16 chains (DEO-SGD$\times$P16) estimates the uncertainty of the centering 9 modes well but fails to deal with the rest of the modes. As to DEO$_{\star}$-SGD$\times$P16, the approximation is rather accurate, as shown in Figure \ref{deo_star_parallel}.




We also present the index process for both schemes in Figure \ref{Swapping_path_chains16}. The vanilla DEO scheme results in volatile paths and a particle takes quite a long time to complete a round trip; by contrast, DEO$_{\star}$ only conducts at most one cheap swap in a window and yields much more deterministic paths. 


% \begin{figure*}[!ht]
%   \centering
%   \vskip -0.05in
%   \subfigure[$\text{DEO}$-SGD$\times$P16]{\includegraphics[width=7cm, height=1.3cm]{figures/NRPT_path_NRPT_iters_20000_chains_16_lr_0.003_0.6_sz_100_swap_rate_0.4_scale_2_window_1_seed_888.png}}\hspace*{0.5em} \subfigure[$\text{DEO}_{\star}$-SGD$\times$P16]{\includegraphics[width=7cm, height=1.3cm]{figures/NRPT_path_NRPT_iters_20000_chains_16_lr_0.003_0.6_sz_100_swap_rate_0.4_scale_2_window_8_seed_888}}
%     \vskip -0.05in
%   \caption{Dynamics of the index process. The red path denotes the round trip path for a particle. }
%   \label{Swapping_path_chains16}
%   \vspace{-0.5em}
% \end{figure*}

% AAAI submission
\begin{figure}[!ht]
  \centering
  % \vskip -0.05in
  \subfigure[$\text{DEO}$-SGD$\times$P16]{\includegraphics[width=8cm, height=1.7cm]{figures/NRPT_path_NRPT_iters_20000_chains_16_lr_0.003_0.6_sz_100_swap_rate_0.4_scale_2_window_1_seed_888.png}}\hspace*{0.5em}\\
  % \vskip -0.05in
  \subfigure[$\text{DEO}_{\star}$-SGD$\times$P16]{\includegraphics[width=8cm, height=1.7cm]{figures/NRPT_path_NRPT_iters_20000_chains_16_lr_0.003_0.6_sz_100_swap_rate_0.4_scale_2_window_8_seed_888}}
    % \vskip -0.05in
  \caption{Dynamics of the index process. The red path denotes the round trip path for a particle. }
  \label{Swapping_path_chains16}
  % \vspace{-0.5em}
\end{figure}



% We run PT-SGD based on 5 processes ($\times$P5) with adaptive learning rates. We set a target swap rate to 0.1 and initialize the learning rates for different chains as 0.01, 0.02, 0.04, 0.08, and 0.16. We fix $\gamma=0.01$. From Figure \ref{multi_modal_simulation}(d), we notice that PT-SGD$\times$P5 approximates the multi-modal distribution very well, \emph{solely by running SGDs with different learning rates and swaps}. To understand why adaptive learning rates facilitates the simulation, we see in Figure \ref{Swapping_path}(a) that the standard geometric initialization of temperatures (achieved by adjusting learning rates) may lead to a small round trip rate because the swap rates are unbalanced among different chains, the top chain yields too few swaps and thus hinders the efficiency. By contrast, we observe in Figure \ref{multi_modal_simulation}(e) that by adaptively adjusting learning rates, we can achieve much more efficient round trips, as demonstrated in Figure \ref{Swapping_path}(b). Eventually, we can better leverage the exploration in high-temperature processes and exploitation in low-temperature processes for accelerating the simulations. 






% \subsection{Posterior approximation and optimization for image data}
\subsection{Posterior approximation for image data}
\label{image_data}
% and test negative log likelihood (NLL), but also compute the expected calibration error (ECE) to measure the credibility of the prediction confidence \citep{temperature_scaling}. 
Next, we conduct experiments on computer vision tasks. We choose ResNet20, ResNet32, and ResNet56 \citep{kaiming15} and train the models on CIFAR100. We report negative log likelihood (NLL) and test accuracy (ACC). For each model, we first pre-train 10 fixed models via 300 epochs and then run algorithms based on momentum SGD (mSGD) for 500 epochs with 10 parallel chains and denote it by DEO$_{\star}$-mSGD$\times$P10. We fix the lowest and highest learning rates as 0.005 and 0.02, respectively. For a fair comparison, we also include the baseline DEO-mSGD$\times$P10 with the same setup except that the window size is 1; the standard ensemble mSGD$\times$P10 is also included with a learning rate of 0.005. In addition, we include two baselines based on a single long chain, i.e. we run stochastic gradient Hamiltonian Monte Carlo \citep{Chen14} 5000 epochs with cyclical learning rates and 50 cycles \citep{ruqi2020} and refer to it as cycSGHMC$\times$T10; we run SWAG$\times$T10 \citep{swag} under similar setups.


In particular for DEO$_{\star}$-mSGD$\times$P10, we tune the target swap rate $\mathbb{S}$ and find an optimum at $\mathbb{S}=0.005$. We compare our proposed algorithm with the four baselines and observe in Table \ref{UQ_test} that  mSGD$\times$P10 can easily obtain competitive results simply through model ensemble \citep{Balaji17}, which outperforms cycSGHMC$\times$T10 and cycSWAG$\times$T10 on ResNet20 and ResNet32 models and perform the worst among the five methods on ResNet56; DEO-\upshape{m}SGD$\times$P10 itself is already a pretty powerful algorithm, however, $\text{DEO}_{\star}$-\upshape{m}SGD$\times$P10 consistently outperforms the vanilla alternative.

\begin{figure}[!ht]
  \centering
  % \vskip -0.1in
  \subfigure[\scriptsize{Round trips}]{\label{cifar_round_trip}\includegraphics[width=1.8cm, height=1.8cm]{figures/cifar100_optimal_window_size.png}}
  \subfigure[\scriptsize{Accuracies}]{\label{cifaar_acc}\includegraphics[width=1.89cm, 
  height=1.8cm]{figures/resnet32_cifar_acc.png}}
  \subfigure[$\eta$]{\label{cifar_learning_rate}\includegraphics[width=1.8cm, height=1.8cm]{figures/resnet32_cifar_lr_corr.png}}
  \subfigure[$\mathbb{S}=0.6$]{\label{cifar_acceptance}\includegraphics[width=1.8cm, height=1.8cm]{figures/resnet32_cifar_acceptance.png}}
    % \vskip -0.1in
  \caption{Study of window sizes, accuracies, learning rates ($\eta$), and acceptance rates ($\mathbb{S}$) on ResNet20.}
  \label{learning_rate_acceptance_rate_v2}
  % \vspace{-0.5em}
\end{figure}

% xxxxxx

To analyze why the proposed scheme performs well, we study the round trips in Figure \ref{cifar_round_trip} and find that the theoretical optimal window obtains around 11 round trips every 100 epochs, which is almost 2 times as much as DEO. In Figure \ref{cifaar_acc}, we observe that the smallest learning rate obtains the highest accuracy (blue) for exploitations, while the largest learning rate yields decent explorations (red); %we see in Figure \ref{cifar_learning_rate} and \ref{cifar_acceptance} that geometrically initialized learning rate fails in producing equi-acceptance, but as the training proceeds, the learning rates converge to fixed points and the acceptance rates for different pairs converge to the target swap rate.
we see in Figure \ref{cifar_learning_rate} and \ref{cifar_acceptance} that geometrically initialized learning rates converge to fixed points and the acceptance rates converge to the target.




% For the visualization of the index process, we observe in Figure \ref{adaptive_path_cifar}(a) that the vanilla DEO scheme leads to volatile trajectories wandering back and forth and is rather inefficient; by contrast, the DEO$_{\star}$ scheme yields well-motivated paths with more deterministic round trips. Interestingly, this path resembles cyclic learning rates \citep{ruqi2020}, which provides a novel viewpoint to \emph{interpret why cyclic learning rates work well empirically}. Nevertheless, the stochastic and parallel manner further improves the margin and eventually leads to efficient approximations.



==> AAAI_2023_Non-reversible_Parallel_Tempering - Clearn_version_for_arXiv (1)/chapters/intro.tex <==
% \vskip -0.1in
\section{Introduction}
% \vskip -0.05in
Langevin diffusion is a standard sampling algorithm that follows a stochastic differential equation
\begin{equation*}
\label{sde}
% \footnotesize
\begin{split}
    d \bbeta_t &= - \nabla U(\bbeta_t) dt+\sqrt{2\tau} d\bW_t,
\end{split}
\end{equation*}
where $\bbeta_t\in\mathbb{R}^d$, $U(\cdot)$ is the energy function $U(\cdot)$, $\bW_t\in\mathbb{R}^d$ is a Brownian motion, and $\tau$ is the temperature. The diffusion process converges to a stationary distribution $\pi(\bbeta)\propto e^{-\frac{U(\bbeta)}{\tau}}$ and setting $\tau=1$ yields a Bayesian posterior. 
A convex $U(\cdot)$ leads to a rapid convergence \citep{dm+16, dk17}; however, a non-convex $U(\cdot)$ inevitably slows down the mixing rate \citep{Maxim17, SVGD, icsgld, awsgld}. To accelerate simulations, replica exchange Langevin diffusion (reLD) proposes to include a high-temperature particle $\bbeta_t^{(P)}$, where $P\in \mathbb{N}^{+} \setminus \{1\}$, for \emph{exploration}. Meanwhile, a low-temperature particle $\bbeta_t^{(1)}$ is presented for \emph{exploitation}:
% PT proposes a high-temperature particle $\bbeta_t^{(P)}$, where $P\in \mathbb{N}^{+} \setminus \{1\}$, for \emph{exploration} and a low-temperature particle $\bbeta_t^{(1)}$ for \emph{exploitation}:
% \begin{equation}
% \label{sde_2_couple}
% % \footnotesize
% \begin{split}
%     d \bbeta_t^{(P)} &= - \nabla U(\bbeta_t^{(P)}) dt+\sqrt{2\tau^{(P)}} d\bW_t^{(P)},\quad d \bbeta_t^{(1)} = - \nabla U(\bbeta_t^{(1)}) dt+\sqrt{2\tau^{(1)}} d\bW_t^{(1)},\\
% \end{split}
% \end{equation}
\begin{equation}
\label{sde_2_couple}
% \footnotesize
\begin{split}
    d \bbeta_t^{(P)} &= - \nabla U(\bbeta_t^{(P)}) dt+\sqrt{2\tau^{(P)}} d\bW_t^{(P)}\\ d \bbeta_t^{(1)} &= - \nabla U(\bbeta_t^{(1)}) dt+\sqrt{2\tau^{(1)}} d\bW_t^{(1)},
\end{split}
\end{equation}
where $\tau^{(P)}>\tau^{(1)}$ and $\bW_t^{(P)}$ is independent of $\bW_t^{(1)}$. To promote more explorations for the low-temperature particle, the particles at the position $(\beta^{(1)}, \beta^{(P)})\in\mathbb{R}^{2d}$ swap with a probability $aS(\beta^{(1)}, \beta^{(P)})$, where 
\begin{equation}
\footnotesize
\label{swap_function}
    S(\beta^{(1)}, \beta^{(P)})= 1\wedge e^{ \big(\frac{1}{\tau^{(1)}}-\frac{1}{\tau^{(P)}}\big)\big( U(\beta^{(1)})- U(\beta^{(P)})\big)},
\end{equation}
and $a\in(0,\infty)$ is the swap intensity. To be specific, the conditional swap rate at time $t$ follows that
\begin{equation*}
\footnotesize
\begin{split}
    \mathbb{P}(\bbeta_{t+dt}&=(\beta^{(P)}, \beta^{(1)})|\bbeta_t=(\beta^{(1)}, \beta^{(P)}))\\
    &=a S(\beta^{(1)}, \beta^{(P)}) d t.
    % \mathbb{P}(\bbeta_{t+dt}=(\beta^{(1)}, \beta^{(P)})|\bbeta_t=(\beta^{(1)}, \beta^{(P)}))&=1-a S(\beta^{(1)}, \beta^{(P)}) d t.\\
\end{split}
\end{equation*}
% \textcolor{red}{FL: Defining $\bbeta_t$ in this way is odd, making $x$ and $\beta$ confusing. 
%  For $U(x)$ and $U(\bbeta)$, which one is to use?}
In the longtime limit, the Markov jump process converges to the joint distribution $\pi(\bbeta^{(1)}, \bbeta^{(P)})\propto e^{-\frac{U(\bbeta^{(1)})}{\tau^{(1)}}-\frac{U(\bbeta^{(P)})}{\tau^{(P)}}}$, where the marginals are denote by $\pi^{(1)}(\bbeta)\propto e^{-\frac{U(\bbeta)}{\tau^{(1)}}}$ and $\pi^{(P)}(\bbeta)\propto e^{-\frac{U(\bbeta)}{\tau^{(P)}}}$.% $\pi^{(1)}(\bbeta)\propto e^{-\frac{U(\bbeta)}{\tau^{(1)}}}$ and $\pi^{(P)}(\bbeta)\propto e^{-\frac{U(\bbeta)}{\tau^{(P)}}}$.% as the \emph{target distribution} and \emph{reference distribution}, respectively.

% \begin{figure*}[!ht]
%   \centering
%   \vskip -0.15in
%   \subfigure[\scriptsize{Reversibility}]
%   {\label{reversible_indx}\includegraphics[width=2.5cm, height=2.5cm]{figures/reversible.png}}\qquad
%   \subfigure[{\scriptsize{Non-reversibility}}]{\label{nonreversible_indx}\includegraphics[width=2.5cm, height=2.5cm]{figures/non-reversibility_v3.png}}\qquad
%     \subfigure[Non-reversible chains]{\label{nonreversible_indx2}\includegraphics[width=6cm, height=2.5cm]{figures/DEO_scheme_v2.png}}\enskip
%     \vskip -0.1in
%   \caption{(Non-)Reversibility. (a): a reversible index that takes $O(P^2)$ time to communicate; (b): a linear non-reversible index moves along a periodic orbit; %, where the dark (light) arrow denotes even (odd) iterations; 
%   (c): non-reversible chains via DEO schemes.}
%   \vskip -0.15in
%   \label{illustration}
% \end{figure*}

\begin{figure*}[!ht]
  \centering
  % \vskip -0.05in
  \subfigure[Reversibility]
  {\label{reversible_indx}\includegraphics[scale=0.27]{figures/reversible.png}}\qquad
  \subfigure[Non-reversibility]{\label{nonreversible_indx}\includegraphics[scale=0.265]{figures/non-reversibility_v3.png}}\qquad
    \subfigure[Non-reversible chains]{\label{nonreversible_indx2}\includegraphics[scale=0.17]{figures/DEO_scheme_v2.png}}\enskip
    % \vskip -0.05in
  \caption{(Non-)Reversibility. (a): a reversible index that takes $O(P^2)$ time to communicate; (b): a linear non-reversible index moves along a periodic orbit; %, where the dark (light) arrow denotes even (odd) iterations; 
  (c): non-reversible chains via DEO schemes.}
  % \vskip -0.05in
  \label{illustration}
\end{figure*}

==> AAAI_2023_Non-reversible_Parallel_Tempering - Clearn_version_for_arXiv (1)/chapters/optimal_NR-PT.tex <==

% \section{Optimal non-reversible scheme for parallel tempering}
\section{Optimal non-reversible scheme for PT}
% \vskip -0.05in
The linear round trip time is appealing for maximizing the algorithmic potential, however, such an advance only occurs given sufficiently many chains. In \emph{non-asymptotic settings} with limited chains, a pearl of wisdom is to avoid frequent swaps \citep{Paul12} and to keep the average acceptance rate from 20\% to 40\% \citep{Kone2005, Martin09, Yves10}. Most importantly, the acceptance rates are severely reduced in big data due to the bias-corrected swaps associated with stochastic energies \citep{deng2020}, see details in section A.1 (appendix) %\ref{reSGLD_appendix}
. As such, maintaining low rejection rates in big data becomes quite challenging and the \emph{issue of quadratic costs} still exists. 

\subsection{Generalized DEO scheme}
Continuing the equi-acceptance settings, we see in Figure \ref{DEO_demo} that the probability for the blue particle to move upward 2 steps to maintain the same momentum after a pair of even and odd iterations is $(1-r)^2$. As such, with a large equi-rejection rate $r$, the blue particle often makes little progress (Figure \ref{illustration_DEO}(b-d)). To handle this issue, the key is to propose small enough rejection rates to track the periodic orbit in Figure \ref{nonreversible_indx}. Instead of pursuing excessive amount of chains, \emph{we resort to a different solution by introducing the generalized even and odd iterations} $E_W$ and $O_W$, where $W\in\mathbb{N}^{+}$, $E_W=\{\lfloor \frac{k}{W}\rfloor \text{ mod } 2 =0|k=1,2,\cdots, \infty\}$ and $O_W=\{\lfloor \frac{k}{W}\rfloor \text{ mod } 2 =1|k=1,2,\cdots, \infty\}$. Now, we present the generalized DEO scheme with a window size $W$ as follows and refer to it as DEO$_W$: \footnote[4]{{The generalized DEO with the optimal window size is denoted by DEO$_{\star}$ and will be studied in the section of Analysis of optimal window size and round trip
time.}}
% \begin{itemize}
%     \item Attempt to swap $E$ (or $O$) pairs at $E_W$ (or $O_W$) iterations.
%     \item Allow \emph{at most one} swap during each cycle of $E_W$ (or $O_W$) iterations.
% \end{itemize}
% \begin{equation}
% \begin{split}
% \label{gDEO}
%     & \circ \text{ Attempt to swap } E \text{ (or } O\text{) pairs at }E_W\text{ (or }O_W\text{) iterations.} \qquad\qquad\qquad\qquad\ \ \\
%     &\circ \text{ Allow }\emph{at most one} \text{ swap during each cycle of } \\
%     &\qquad E_W \text{ (or }O_W\text{) iterations.}
% \end{split}
% \end{equation}
\begin{equation*}
% \footnotesize
\begin{split}
% \label{gDEO}
    & \footnotesize{\circ \text{ Attempt to swap } E \text{ (or } O\text{) pairs at }E_W\text{ (or }O_W\text{) iterations.}} \qquad\qquad\qquad\qquad\ \ \\
    & \footnotesize{\circ \text{ Allow }\emph{at most one} \text{ swap at }  E_W \text{ (or }O_W\text{) iterations.}}
\end{split}
\end{equation*}
As shown in Figure \ref{DEO2_demo}, the blue particle has a larger chance of $(1-r^2)^2$ to move upward 2 steps given $W=2$ instead of $(1-r)^2$ when $W=1$, although the window number is also halved. Such a trade-off inspires us to analyze the expected round trip time based on the window of size $W$.

\paragraph{How to alleviate the bias} Although allowing at most one swap introduces the geometric stopping of swaps and affects the target distribution (see section 2 of \citep{geo_stop_random_walk}), the bias can be much alleviated empirically by introducing a window-wise correction term. Moreover, it becomes rather mild when the energy estimators have a large variance. Check section C.2 (appendix) %\ref{approx_upper_bound} 
for the details. For tasks without high-accuracy demands, we propose to ignore the correction term in practice following \citet{Li16} to facilitate the round trip analysis and promote more tractable explorations.


% \begin{figure*}[!ht]
%   \centering
% %   \vskip -0.05in
%   \subfigure[$\sigma=2$]{\label{pt_sd_2}\includegraphics[width=3.3cm, height=3.3cm]{figures/window_correction/sd_2.png}}
%   \subfigure[$\sigma=3$]{\label{pt_sd_3}\includegraphics[width=3.3cm, height=3.3cm]{figures/window_correction/sd_3.png}}
%   \subfigure[$\sigma=4$]{\label{pt_sd_4}\includegraphics[width=3.3cm, height=3.3cm]{figures/window_correction/sd_4.png}}
%   \subfigure[$\sigma=5$]{\label{pt_sd_5}\includegraphics[width=3.3cm, height=3.3cm]{figures/window_correction/sd_5.png}} \\
%   \subfigure[$\sigma=2$]{\label{pt_sd_2_corr}\includegraphics[width=3.3cm, height=3.3cm]{figures/window_correction/sd_2_corr.png}}
% \subfigure[$\sigma=3$]{\label{pt_sd_3_corr}\includegraphics[width=3.3cm, height=3.3cm]{figures/window_correction/sd_3_corr.png}}
%   \subfigure[$\sigma=4$]{\label{pt_sd_4_corr}\includegraphics[width=3.3cm, height=3.3cm]{figures/window_correction/sd_4_corr.png}}
%   \subfigure[$\sigma=5$]{\label{pt_sd_5_corr}\includegraphics[width=3.3cm, height=3.3cm]{figures/window_correction/sd_5_corr.png}}
%     \vskip -0.05in
%   \caption{Simulations of the multi-modal distribution through different sampling algorithms. }
%   \label{bias_with_without_correction}
%   \vspace{-0.5em}
% \end{figure*}



% The round trip time is hard to analyze due to the non-Markovian index process. To simplify the analysis, we follow \citet{Syed_jrssb} and treat swap indicators as independent Bernoulli variables.


\subsection{Analysis of round trip time}
\label{main_round_trip_analysis}

To bring sufficient interactions between the reference distribution $\pi^{(P)}$ and the target distribution $\pi^{(1)}$, we expect to minimize the expected round trip time $T$ (defined in section A.5 (appendix) %\ref{others}
) to ensure both efficient exploitation and explorations. The non-Markovian nature of the index process makes the analysis challenging. To facilitate the analysis, we treat swap indicators as independent Bernoulli variables following \citet{Syed_jrssb}. Combining the Markov property, we estimate the expected round trip time $\hE[T]$ as follows:
\begin{lemma}
\label{thm:round_trip_time}
Under the stationary and weak independence assumptions B1 and B2 in section B (appendix) %\ref{analysis_of_round_trip}
, for $P$ ($P\ge 2$) chains with window size $W$ ($W\ge 1$) and rejection rates $\{r_p\}_{p=1}^{P-1}$, we have
\begin{align} \label{eq:RTT_main}
{\hE[T]=2WP+\underbrace{2WP\sum_{p=1}^{P-1}\frac{r_p^W}{1-r_p^W}}_{\text{Quadratic term in }P}}.
\end{align}
\end{lemma}
The proof in section B.1 %\ref{analyze_round_trip}
shows that $\E[T]$ increases as we adopt larger number of chains $P$ and rejection rates $\{r_p\}_{p=1}^{P-1}$. In such a case, the round trip rate $\frac{P}{\hE[T]}$ is also maximized by the key renewal theorem. In particular, applying $W=1$ recovers the vanilla DEO scheme.

\subsection{Analysis of optimal window size and round trip time}
\label{windiw_size_round_trip}
By Lemma \ref{thm:round_trip_time}, we observe a potential to remove the quadratic term given an appropriate $W$. Such a fact motivates us to study the optimal $W$ to achieve the best efficiency. Under the equi-acceptance settings, by treating $W$ as a continuous variable and taking the derivative with respect to $W$, we have
\begin{equation} \label{eq:dWRTT_main}
\begin{split}
\frac{\partial}{\partial W}\hE[T]&=\frac{2P}{(1-r^W)^2}\bigg\{(1-r^W)^2 \\
&+(P-1)r^W(1-r^W+W\log r)\bigg\},
\end{split}
\end{equation}
where $r$ is the equi-rejection rate for adjacent chains. Define $x:=r^W\in(0, 1)$, where $W=\log_r(x)=\frac{\log x}{\log r}$. The following analysis hinges on the study of the solution of $g(x)=(1-x)^2+(P-1)x(1-x+\log(x))=0$. By analyzing the growth of derivatives and boundary values, we can identify the \emph{uniqueness} of the solution. Then, we proceed to verify that $\frac{1}{P\log P}$ yields an asymptotic approximation such that $g(\frac{1}{P\log P})=-\frac{\log(\log P)}{\log P}+O\left(\frac{1}{\log P}\right)\rightarrow 0$ as $P\rightarrow \infty$. In the end, we have


\begin{theorem} \label{col:W_approx}
Under Assumptions B1 (Stationarity) and B2 (Weak independence) based on equi-acceptance settings, if $P=2,3$, the minimal round trip time is achieved when $W=1$. If $P\ge 4$, with the optimal window size $W_{\star}\approx\left\lceil\frac{\log P+\log\log P}{-\log r}\right\rceil$, where $\lceil\cdot\rceil$ is the ceiling function. The round trip time follows $O(\frac{P\log P}{-\log r})$. % and the round trip rate is at least $\Omega(\frac{-\log r}{\log P})$. 
\end{theorem}

The above result yields a remarkable round trip time of $O(P\log P)$ by setting the optimal window size $W_{\star}$. By contrast, the vanilla DEO scheme only leads to a longer time of $O(P^2)$ \footnote[4]{By Taylor expansion, given a large rejection rate $r$, $-\log(r)=1-r$, which means $\frac{1}{-\log(r)}=O(\frac{r}{1-r})$.}. Denoting by $\text{DEO}_{\star}$ the generalized DEO scheme with the optimal window size $W_{\star}$, we summarize the popular swap schemes in Table \ref{round_trip_time_cost}, where the DEO$_{\star}$ scheme performs the best among all the three criteria. We acknowledge that the assumptions are inevitably strong to simplify the analysis \citep{Syed_jrssb} due to the intractable index process. Empirically, assumption B1 approximately holds after a sufficient burn-in period; more in-depth discussions on the robustness of assumption B2 have also been evaluated in section 7.2 of \citet{Syed_jrssb}.


\begin{table*}[ht]
\begin{sc}
% \vspace{-0.05in}
\caption[Table caption text]{{Round trip time and swap time for different schemes. Notably, non-asymptotic refers to cases with large rejection rates due to a limited number of chains; asymptotic occurs given sufficiently many chains such that rejection rates are close to 0. The APE scheme requires an expensive swap time of $O(P^3)$ and is not compared. }} \label{round_trip_time_cost}
% \small
\begin{center} 
\begin{tabular}{c|cccc}
\hline
 & \textbf{\footnotesize{Round trip time} \scriptsize{(non-asymptotic)}} & \footnotesize{Round trip time} \scriptsize{(asymptotic)} & \footnotesize{Swap time} \\
\hline
ADJ & $O(P^2)$ \scriptsize{\citep{Nadler07}} & $O(P^2)$ \scriptsize{\citep{Nadler07}} & $O(P)$ \\
SEO & $O(P^2)$ \scriptsize{\citep{Syed_jrssb}} & $O(P^2)$ \scriptsize{\citep{Syed_jrssb}} & \bm{$O(1)$} \\
DEO & $O(P^2)$ \scriptsize{\citep{Syed_jrssb}} & \bm{$O(P)$} \scriptsize{\citep{Syed_jrssb}}  & \bm{$O(1)$} \\
\hline
${\text{DEO}_{\star}}$  & $\bm{O(P\log P)}$ & \bm{$O(P)$}  & \bm{$O(1)$} \\
%\upshape{g}
\hline
\end{tabular}
\end{center}
\end{sc}
% \vspace{-0.05in}
\end{table*}

% \textcolor{red}{FL: since $W$ increases with $P$, the swap time should be a function of $W$ (making many tries). It might not be O(1). Please double check this.}


\subsection{Discussions on the optimal number of chains}
\label{main_optimal_chain}


Note that in practice given $P$ parallel chains, a large $P$ leads to a smaller equi-rejection rate $r$. As such, we can further obtain a crude estimate of the optimal $P$ to minimize the round trip time.
\begin{corollary} \label{col:P_approx}
Under Assumptions B1-B4 and C1 under equi-acceptance settings with the optimal window size, the optimal chains follow that $P_{\star}> \min_p \frac{\sigma_p}{3\tau^{(p)}} \log(\frac{\tau^{(P)}}{\tau^{(1)}})$, where $\sigma_p$ is defined in Eq.(14) (appendix) %(\ref{sigma_p})
.
\end{corollary}
The assumptions and proof are postponed in section B.3 (appendix) %\ref{opt_num_chains}
. In mini-batch settings, insufficient chains may lead to few effective swaps for accelerations; by contrast, introducing too many chains may be too costly in terms of the round trip time. This is different from the conclusion in full-batch settings, where \citet{Syed_jrssb} suggested running the vanilla DEO scheme with as many chains as possible to yield a small enough equi-rejection rate $r$ to maintain the non-reversibility. 

\paragraph{Cutoff phenomenon} On the one hand, when we only afford at most $P$ chains, where $P< P_{\star}$, a large equi-rejection rate $r$ is inevitable and DEO$_{\star}$ is preferred over DEO; on the other hand, the rejection rate $r$ goes to $0$ when $P\gg P_{\star}$ and DEO$_{\star}$ recovers the DEO scheme. 

In section B.4 (appendix) %\ref{estimate_p_star}
, we show that $P_{\star}$ is in the \emph{order of thousands} for the CIFAR100 example, which is hard to achieve due to the limited computational budget and further motivates us to adopt finite chains with a target swap rate $\mathbb{S}$ to balance between acceleration and accuracy.

\begin{algorithm}[tb]
  \small
  % \vskip -0.03in
  \caption{Non-reversible parallel tempering with SGD-based exploration kernels (DEO$_{\star}$-SGD).}
  \label{alg}
\begin{algorithmic}
\STATE{\textbf{Input} Number of chains $P\geq 3$, boundary learning rates $\eta^{(1)}$ and $\eta^{(P)}$, target swap rate $\mathbb{S}$.}
\STATE{\textbf{Input} Optimal window size $W:=\left\lceil \frac{\log P + \log\log P}{-\log(1-\mathbb{S})}\right\rceil$, total iterations $K$, and step sizes $\{\gamma_{k}\}_{k=0}^K$.}

\FOR{ $k=0$ \text{ to } $K$ } 
    \STATE{$\bbeta_{k+1}\sim \mathcal{T}_{\eta}(\bbeta_{k})$ following Eq.(\ref{pt_sgd}) 
     \quad$\triangleright$ \textcolor{blue}{Sampling phase}
    }
    
    \STATE{$\mathcal{P}=\big\{\forall p\in\{1, 2,\cdots, P\}: p \text{ mod } 2 = \lfloor \frac{k}{W}\rfloor \text{ mod } 2\big\}$.}
    
    
    

    \FOR{ $p=1,2$ \text{ to } $P-1$ }
        \STATE{$\mathcal{A}^{(p)}:=1_{\widetilde U( \bbeta_{k+1}^{(p+1)})+\mathbb{C}_k<\widetilde U( \bbeta_{k+1}^{(p)})}$}
        

        \IF{k\text{ mod } W=0}
        \STATE{\emph{Open: }$\mathcal{G}^{(p)}=1$. \quad $\triangleright$ 
        \textcolor{blue}{Open the gate to allow swaps}}
        \ENDIF
        % \STATE{$\mathcal{G}^{(p)}:=1_{k\text{ mod } W=0}$. \qquad\ \  $\triangleright$ Open the gate to allow swaps}
        
        \IF{$p\in \mathcal{P}$ \text{ and } $\mathcal{G}^{(p)}$ \text{ and } $\mathcal{A}^{(p)}$}
        
        
        
        
        \STATE{\emph{Swap: } $ \bbeta_{k+1}^{(p)}$ and $ \bbeta_{k+1}^{(p+1)}$. \ \ $\triangleright$ \textcolor{blue}{Communication phase}}
        \STATE{ \emph{Freeze: } $\mathcal{G}^{(p)} = 0.$   $\triangleright$ \textcolor{blue}{Close the gate to refuse swaps}}
        \ENDIF
        \IF{$p>1$}
        \STATE{\emph{Update learning rate (temperature) following Eq.(\ref{double_SA})}}
        \ENDIF
    \ENDFOR
    
    \STATE{\emph{Correction: } $\mathbb{C}_{k+1}=\mathbb{C}_k+\gamma_{k}\left(\frac{1}{P-1}\sum_{p=1}^{P-1} \mathcal{A}^{(p)}-\mathbb{S}\right).$}
\ENDFOR
\STATE{\textbf{Output } Target models $\{\bbeta_{k}^{(1)}\}_{k=1}^{K}$.}
% \vskip -0.15in
\end{algorithmic}
\end{algorithm}

==> AAAI_2023_Non-reversible_Parallel_Tempering - Clearn_version_for_arXiv (1)/chapters/prelim.tex <==
% \vskip -0.1in
\section{Preliminaries}
% \vskip -0.1in
Achieving sufficient explorations requires a large $\tau^{(P)}$, which leads to limited accelerations due to a \emph{small overlap} between $\pi^{(1)}$ and $\pi^{(P)}$. To tackle this issue, one can bring in multiple particles with temperatures $(\tau^{(2)}, \cdots, \tau^{(P-1)})$, where $\tau^{(1)}<\tau^{(2)}<\cdots <\tau^{(P)}$, to hollow out ``tunnels''. To  maintain feasibility, numerous schemes are presented to select candidate pairs to attempt the swaps. 
% \vskip -0.1in
\paragraph{APE} The all-pairs exchange (APE) attempts to swap arbitrary pair of chains \citep{Brenner07, Martin09}, %which shows remarkable efficiency given low acceptance rates \citep{Martin09}. 
however, such a method requires a swap time (see definition in section A.5 (appendix) %\ref{others}
) of $O(P^3)$  and may not be user-friendly in practice.

% \vskip -0.1in
\paragraph{ADJ} In addition to swap arbitrary pairs, one can also swap \emph{adjacent} (ADJ) pairs iteratively from $(1,2)$, $(2,3)$, to $(P-1,P)$ under the Metropolis rule. Despite the convenience, the \emph{sequential nature} requires to wait for exchange information from previous exchanges, which only works well with a small number of chains and has greatly limited its extension to a multi-core or distributed context.
% \vskip -0.05in
\paragraph{SEO} The stochastic even-odd (SEO) scheme first divides the adjacent pairs $\{(p-1, p)|p=2,\cdots, P\}$ into $E$ and $O$, where $E$ and $O$ denote even and odd pairs of forms $(2p-1, 2p)$ and $(2p, 2p+1)$, respectively. Then, SEO randomly picks $E$ or $O$ pairs with an equal chance in each iteration to attempt the swaps. Notably, it can be conducted \emph{simultaneously} without waiting from other chains. The scheme yields a reversible process (see Figure \ref{reversible_indx}), however, the gains in overcoming the sequential obstacle don't offset the \emph{$O(P^2)$ round trip time} and SEO is still not effective enough.
% \vskip -0.05in

\begin{figure*}[!ht]
  \centering
  % \vskip -0.05in
  \subfigure[DEO]{\label{DEO_demo}\includegraphics[width=2.4cm, height=1.8cm]{figures/DEO_good.png}}\qquad
  \subfigure[Bad case 1]{\includegraphics[width=2.4cm, height=1.8cm]{figures/DEO_bad_1.png}}\qquad
  \subfigure[Bad case 2]{\includegraphics[width=2.4cm, height=1.8cm]{figures/DEO_bad_2.png}}\qquad
  \subfigure[Bad case 3]{\includegraphics[width=2.4cm, height=1.8cm]{figures/DEO_bad_3.png}}\qquad
  \subfigure[$\text{DEO}_2$]{\label{DEO2_demo}\includegraphics[width=3.7cm, height=1.8cm]{figures/gDEO.png}}\qquad
    % \vskip -0.05in
  \caption{Illustration of DEO and DEO$_2$. (a): an ideal DEO scheme; (b-d): failed DEO swaps given a large $r$; (e): how DEO$_2$ tackles the issue. The x-axis and y-axis denote (generalized) $E$ (or $O$) iterations and $E$ (or $O$) pairs, respectively. The dashed line denotes no swap; the gray areas are frozen to refuse swapping odd pairs at even iterations (or vice versa); the blue area freezes swap attempts.}
  % \vskip -0.05in
  \label{illustration_DEO}
\end{figure*}
% \vskip -0.05in
\paragraph{DEO} The deterministic even-odd (DEO) scheme instead attempts to swap even ($E$) pairs at even ($E$) iterations and odd ($O$) pairs at odd ($O$) iterations alternatingly\footnote[2]{{$E$ ($O$) shown in iterations means even (odd) iterations and denotes even (odd) pairs for chain indexes.}} \citep{DEO}. The asymmetric manner was later interpreted as a non-reversible PT \citep{Syed_jrssb} and an ideal index process follows a periodic orbit, as shown in Figure \ref{nonreversible_indx}. With a large swap rate, Figure \ref{nonreversible_indx2} shows how the scheme yields an almost straight path and a linear round trip time can be expected.
% \vskip -0.05in
\paragraph{Equi-acceptance} The power of PT hinges on maximizing the number of round trips, which is equivalent to minimizing $\sum_{p=1}^{P-1} \frac{1}{1-r_p}$ \citep{Nadler07_V2}, where $r_p$ denotes the rejection rate for the chain pair $(p, p+1)$. Moreover, $\sum_{p=1}^{P-1} r_p$ converges to a fixed barrier $\Lambda$ as $P\rightarrow \infty$ \citep{Predescu04, Syed_jrssb}. Applying Lagrange multiplies to the constrained optimization problem leads to $r_1=r_2=\cdots=r_{P-1}:=r$, where $r$ is the \emph{equi-rejection rate}. In general, a quadratic round trip time is required for ADJ and SEO due to the reversible indexes. By contrast, DEO only yields a \emph{linear round trip} time in terms of $P$ as $P\rightarrow \infty$ \citep{Syed_jrssb}.


==> AAAI_2023_Non-reversible_Parallel_Tempering - Clearn_version_for_arXiv (1)/chapters/user_friendly_approximation.tex <==

\section{User-friendly approximate explorations in big Data}
% \vskip -0.05in


Despite the asymptotic correctness, stochastic gradient Langevin dynamics \citep{Welling11} (SGLD) only works well given \emph{small enough learning rates} and fails in explorative purposes \citep{Ahn12}. A large learning rate, however, leads to excessive stochastic gradient noise and ends up with a crude approximation. As such, similarly to \citet{SWA1, ruqi2020}, we only adopt SGLD for exploitations.

Efficient explorations not only require a high temperature but also prefer a large learning rate. Such a demand inspires us to consider SGD with a constant learning rate $\eta$ as the exploration component
\begin{equation}
\begin{split}\label{sgd_approx}
\footnotesize
    \bbeta_{k+1} &=\bbeta_{k} - \eta \nabla \widetilde U(\bbeta_k)=\bbeta_{k} - \eta(\nabla U(\bbeta_k)+\varepsilon(\bbeta_k))\\
    &=\bbeta_{k} - \eta\nabla U(\bbeta_k)-\sqrt{2\eta \big(\frac{\eta}{2}\big)}\varepsilon(\bbeta_k),
\end{split}
\end{equation}
where $\widetilde U(\cdot)$ is the unbiased energy estimate of $U(\cdot)$ and  $\varepsilon(\bbeta_k)\in\mathbb{R}^d$ is the stochastic gradient noise with mean 0. Under mild normality assumptions on $\varepsilon$ \citep{Mandt, SGD_AOS}, $\bbeta_{k}$ converges approximately to an invariant distribution, where the underlying \emph{temperature linearly depends on the learning rate $\eta$}. Motivated by this fact, we propose an approximate transition kernel $\mathcal{T}_{\eta}$ with $P$ parallel \emph{SGD runs} based on different learning rates
\begin{equation}  
\begin{split}
\footnotesize
\label{pt_sgd}
\textbf{Exploration: }\left\{  
             \begin{array}{lr}  
             \footnotesize{\small{\bbeta_{k+1}^{(P)}=\bbeta_{k}^{(P)} - \eta^{(P)}\nabla \widetilde U(\bbeta_k^{(P)})}}, \\  
              \\
              \footnotesize{\cdots}  \\
             \footnotesize{\bbeta_{k+1}^{(2)} =\bbeta_{k}^{(2)} - \eta^{(2)}\nabla \widetilde U(\bbeta_k^{(2)})},\\
             \end{array}
\right. \qquad\qquad\qquad\qquad\  & \\
\textbf{Exploitation: } \ \quad\footnotesize{\bbeta_{k+1}^{(1)}=\bbeta_{k}^{(1)} - \eta^{(1)}\nabla \widetilde U(\bbeta_k^{(1)})\ \ +\overbrace{\Xi_k}^{\text{optional}},\qquad\qquad\quad\quad}\ &\\
\end{split}
\end{equation}
where $\eta^{(1)}<\eta^{(2)}<\cdots<\eta^{(P)}$, $\Xi_k\sim \mathcal{N}(0, 2\eta^{(1)}\tau^{(1)})$, and $\tau^{(1)}$ is the target temperature.

% \textcolor{red}{FL: Is $\tau^{(1)}$ smaller than $\eta^{(2)}/2$? Should this be ensured? Otherwise, the scheme will not comply with the idea of parallel tempering. } \Wei{this part is hard to justify since the stochastic gradient scale is hard to control.}

Since there exists an optimal learning rate for SGD to estimate the desired distribution through Laplace approximation \citep{Mandt}, the exploitation kernel can be also replaced with SGD based on constant learning rates if the accuracy demand is not high. Regarding the validity of adopting different learning rates for parallel tempering, we leave discussions to section A.2 (appendix) %\ref{diff_lr}
. 


\subsection{Approximation analysis}
Moreover, the stochastic gradient noise exploits the Fisher information \citep{Ahn12, zhanxing_anisotropic, Chaudhari17} and yields convergence potential to wide optima with good generalizations \citep{Berthier, difan_2021}. Despite the implementation convenience, the inclusion of SGDs has made the temperature variable inaccessible, rendering a difficulty in implementing the Metropolis rule Eq.(\ref{swap_function}). To tackle this issue, we utilize the randomness in stochastic energies and propose a \emph{deterministic swap condition} for the approximate kernel $\mathcal{T}_{\eta}$ in Eq.(\ref{pt_sgd}) 
% \begin{equation}
% \small
% \begin{split}
%     \label{deterministic_swap}
%     &\textbf{Deterministic swap condition: }\\
%     &\quad\footnotesize{(\bbeta^{(p)}, \bbeta^{(p+1)})\rightarrow (\bbeta^{(p+1)}, \bbeta^{(p)}) \text{ if } \widetilde U(\bbeta^{(p+1)})+\mathbb{C}<\widetilde U(\bbeta^{(p)})},
% \end{split}
% \end{equation}
\begin{equation}
\small
\begin{split}
    \label{deterministic_swap}
    &\textbf{Deterministic swap condition: } \text{ if } \widetilde U(\bbeta^{(p+1)})+\mathbb{C}<\widetilde U(\bbeta^{(p)})\\
    &\quad\qquad\qquad\footnotesize{(\bbeta^{(p)}, \bbeta^{(p+1)})\rightarrow (\bbeta^{(p+1)}, \bbeta^{(p)}) },
\end{split}
\end{equation}
where $p\in\{1,2,\cdots, P-1\}$, $\mathbb{C}>0$ is a correction buffer to approximate the Metropolis rule Eq.(\ref{swap_function}). 


\begin{lemma}\label{thres_approx} Assume the energy normality assumption (C1), then for any fixed $\partial U_p:=U(\bbeta^{(p)})- U(\bbeta^{(p+1)})$, there exists an optimal $\mathbb{C}_{\star}\in (0, (\frac{1}{\tau^{(p)}}-\frac{1}{\tau^{(p+1)}})\sigma_p^2]$  that perfectly approximates the random event $\widetilde S(\bbeta^{(p)}, \bbeta^{(p+1)})>u$, where $\sigma_p$ defined in Eq.(14) (appendix) %(\ref{sigma_p}) 
and $u\sim\text{Unif}\ [0, 1]$.
\end{lemma}

The proof is postponed in section C.1 (appendix) % \ref{gap_bet_acc_rate}
, which paves the way for the guarantee that a \emph{deterministic swap condition} may replace the Metropolis rule Eq.(\ref{swap_function}) for approximations. In addition, the normality assumption can be naturally extended to the asymptotic normality assumption \citep{Matias19, deng_VR} given large enough batch sizes.  

Admittedly, the approximation error still exists for different $\partial U_p$. By the mean-value theorem, there exists a tunable $\mathbb{C}$ to optimize the overall approximation. Further invoking the central limit theorem such that $\varepsilon(\cdot)$ in Eq.(\ref{sgd_approx}) approximates a Gaussian distribution with a fixed covariance, we can expect a bounded approximation error for the SGD-based exploration kernels \citep{Mandt}.

\begin{theorem}\label{bound_approx}
Consider the exact transition kernel $\mathcal{T}$ and the proposed approximate kernel $\mathcal{T}_{\eta}$, %(\textcolor{red}{ FL: $\mathcal{T}_{\eta}$ needs to be defined. }, 
which yield stationary distributions $\pi$ and $\pi_{\eta}$, respectively. Under smoothness (C2) and dissipativity assumptions (C3) \citep{mattingly02, Maxim17, Xu18}, $\mathcal{T}$ satisfies the geometric ergodicity such that there is a contraction constant $\rho\in [0, 1)$ for any distribution $\mu$:
\begin{equation*}
    \|\mu\mathcal{T}-\pi\|_{\text{TV}}\leq \rho \|\mu-\pi\|_{\text{TV}},
\end{equation*}
where $\|\cdot\|_{\text{TV}}$ is the total variation (TV) distance. Moreover, assume that $\varepsilon(\cdot)\sim\mathcal{N}(0, \mathcal{M})$ for some positive definite matrix $\mathcal{M}$ (C4) \citep{Mandt}, then there is a uniform upper bound of the one step error between $\mathcal{T}$ and $\mathcal{T}_{\eta}$ such that 
\begin{equation*}
    \|\mu\mathcal{T}-\mu\mathcal{T}_{\eta}\|_{\text{TV}}\leq \Delta_{\max}, \forall \mu,
\end{equation*}
where $\Delta_{\max}\geq 0$ is a constant. Eventually, the TV distance between $\pi$ and $\pi_{\eta}$ is bounded by
\begin{equation*}
    \|\pi-\pi_{\eta}\|_{\text{TV}}\leq \frac{\Delta_{\max}}{1-\rho}.
\end{equation*}
\end{theorem}

The proof is postponed to section C.2 (appendix) %\ref{approx_upper_bound}
. The SGD-based exploration kernels \emph{no longer require to fine-tune the temperatures} directly and naturally inherits the empirical successes of SGD in large-scale deep learning tasks. The inaccessible Metropolis rule Eq.(\ref{swap_function}) is approximated via the \emph{deterministic swap condition} Eq.(\ref{deterministic_swap}) and leads to robust approximations by \emph{tuning $\bm{\eta}=(\eta^{(1)},\cdots, \eta^{(P)})$ and $\mathbb{C}$}. 

In addition, our proposed algorithm for posterior approximation also relates to non-convex optimization. For detailed discussions, we refer interested readers to section A.4 (appendix) %\ref{connection_2_non_convex}
.

\subsection{Equi-acceptance parallel tempering on optimized paths}

Stochastic approximation (SA) is a standard method to achieve equi-acceptance \citep{Yves10, Miasojedow_2013}, however, implementing this idea with fixed $\eta^{(1)}$ and $\eta^{(P)}$ is rather non-trivial. Motivated by the linear relation between learning rate and temperature, we propose to adaptively \emph{optimize the learning rates} to achieve equi-acceptance in a user-friendly manner. Further by the geometric temperature spacing commonly adopted by practitioners \citep{Kofke02, parallel_tempering05, Syed_jrssb}, we adopt the following scheme on a \emph{logarithmic scale}
\begin{equation}
\label{sa_exp}
    \partial \log(\upsilon_t^{(p)})=h^{(p)}(\upsilon_t^{(p)}),
\end{equation}
where $p\in\{1,2,\cdots, P-1\}$, $\upsilon_t^{(p)}=\eta_t^{(p+1)}-\eta_t^{(p)}$, $h^{(p)}(\upsilon_t^{(p)}):=\int H^{(p)}(\upsilon_k^{(p)}, \bbeta) \pi^{(p, p+1)}(d\bbeta)$ is the mean-field function, $\pi^{(p, p+1)}$ is the joint invariant distribution for the $p$-th and $p+1$-th processes.  In particular, $H^{(p)}(\upsilon_k^{(p)}, \bbeta)=1_{\widetilde U( \bbeta^{(p+1)})+\mathbb{C}<\widetilde U( \bbeta^{(p)})}-\mathbb{S}$ is the random-field function to approximate $h^{(p)}(\upsilon_k^{(p)})$ with limited perturbations, $\upsilon_k^{(p)}$ \footnote[2]{$\upsilon_t^{(p)}$ denotes a continuous-time diffusion at time $t$ and $\upsilon_k^{(p)}$ is a discrete approximation at iteration $k$.} implicitly affects the distribution of the indicator function, and $\mathbb{S}$ is the target swap rate.  Now consider stochastic approximation of Eq.(\ref{sa_exp}), we have
\begin{equation}
\label{sa_exp_euler}
    \log(\upsilon_{k+1}^{(p)})=\log(\upsilon_{k}^{(p)}) + \gamma_k H^{(p)}(\upsilon_k^{(p)}, \bbeta_k),
\end{equation}
where $\gamma_k$ is the step size. Reformulating Eq.(\ref{sa_exp_euler}), we have
\begin{equation*}
\label{sa_exp_taylor}
    \upsilon_{k+1}^{(p)} = \max(0, \upsilon_{k}^{(p)})e^{\gamma_k H(\upsilon_k^{(p)})},
\end{equation*}
where the $\max$ operator is conducted explicitly to ensure the sequence of learning rates is non-decreasing. This means given fixed boundary learning rates (temperatures) $\eta_k^{(p-1)}$ and $\eta_k^{(p+1)}$, applying $\eta^{(p)}=\eta^{(p-1)}+\upsilon^{(p)}$ and $\eta^{(p)}=\eta^{(p+1)}-\upsilon^{(p+1)}$ for $p\in\{2,3,\cdots, P-1\}$ lead to
\begin{equation}
\begin{split}
    \label{double_SA_forward_backward}
    \eta_{k+1}^{(p)}&=\underbrace{\eta_k^{(p-1)}+ \max(0, \upsilon_{k}^{(p)})e^{\gamma_k H(\upsilon_k^{(p)})}}_{\text{forward sequence}}\\
    &=\underbrace{\eta_k^{(p+1)}- \max(0, \upsilon_{k}^{(p+1)})e^{\gamma_k H(\upsilon_k^{(p+1)})}}_{\text{backward sequence}}.
\end{split}
\end{equation}



\paragraph{Adaptive learning rates (temperatures)} Now given a fixed $\eta^{(1)}$, the sequence $\eta^{(2)}$, $\eta^{(3)}$, $\cdots$, $\eta^{(P)}$ can be approximated iteratively via the forward sequence of (\ref{double_SA_forward_backward}); conversely, given a fixed $\eta^{(P)}$, the backward sequence $\eta^{(P-1)}$, $\eta^{(P-2)}$, $\cdots$, $\eta^{(1)}$ can be decided reversely as well. Combining the forward and backward sequences, $\eta_{k+1}^{(p)}$ can be approximated via 
\begin{equation}
\small
\begin{split}
    \label{double_SA}
    &\eta_{k+1}^{(p)}:=\frac{\eta_k^{(p-1)}+\eta_k^{(p+1)}}{2}+\\
    &\frac{\max(0, \upsilon_{k}^{(p)})e^{\gamma_k H(\upsilon_k^{(p)})} - \max(0, \upsilon_{k}^{(p+1)})e^{\gamma_k H(\upsilon_k^{(p+1)})}}{2},
\end{split}
\end{equation}
which resembles the \emph{binary search} in the SA framework. In particular, the first term is the middle point given boundary learning rates and the second term continues to penalize learning rates that violates the equi-acceptance between pairs $(p-1, p)$ and $(p, p+1)$ until an equilibrium is achieved. 

This is the first attempt to achieve equi-acceptance given two fixed boundary values to our best knowledge. By contrast, \citet{Syed_jrssb} proposed to estimate the barrier $\Lambda$ to determine the temperatures and it easily fails in big data given a finite number of chains and bias-corrected swaps.  

% \Wei{distinguish nominal swap rate and real swap rate}

\paragraph{Adaptive correction buffers} In addition, equi-acceptance does not guarantee a convergence to the desired  acceptance rate $\mathbb{S}$. To avoid this issue, we propose to adaptively optimize $\mathbb{C}$ as follows
\begin{equation}\label{unknown_threhold}\small
    \mathbb{C}_{k+1}=\mathbb{C}_k+\gamma_k\left(\frac{1}{P-1}\sum_{p=1}^{P-1} 1_{\widetilde U( \bbeta_{k+1}^{(p+1)})+\mathbb{C}_k-\widetilde U( \bbeta_{k+1}^{(p)})<0}-\mathbb{S}\right).
\end{equation}






As $k\rightarrow \infty$, the threshold and the adaptive learning rates converge to the desired fixed points. Note that setting a uniform $\mathbb{C}$ greatly simplifies the algorithm.%; in more delicate cases, problem-specific rules are also recommended.
Now we refer to the approximate non-reversible parallel tempering algorithm with the DEO$_{\star}$ scheme and SGD-based exploration kernels as DEO$_{\star}$-SGD and formally formulate our algorithm in Algorithm \ref{alg}. Extensions of SGD with a preconditioner \citep{Li16} or momentum \citep{Chen14} to further improve the approximation and efficiency are both straightforward \citep{Mandt} and are denoted as DEO$_{\star}$-pSGD and DEO$_{\star}$-mSGD, respectively.

% NIPS submission
% \begin{figure*}[!ht]
%   \centering
%   \vskip -0.07in
%   \subfigure[{Ground truth} ]{\label{multi_density_truth}\includegraphics[width=2.2cm, height=2.2cm]{figures/ground_truth_NRPT_iters_20000_chains_16_lr_0.01_0.5_sz_100_swap_rate_0.4_scale_2_window_8_seed_8.png}}\quad
%   \subfigure[{SGLD$\times$P16}]{\label{sgld_parallel}\includegraphics[width=2.2cm, height=2.2cm]{figures/NRPT_density_sgld_ensemble_iters_20000_chains_16_lr_0.003_0.6_sz_100_swap_rate_0.4_scale_2_window_8_seed_888.png}}\quad
%   \subfigure[\scriptsize{cycSGLD$\times$T16}]{\label{cycSGLD_parallel}\includegraphics[width=2.2cm, height=2.2cm]{figures/NRPT_density_cyclic_sgld_iters_20000_chains_16_lr_0.003_0.6_sz_100_swap_rate_0.4_scale_2_window_8_seed_888.png}}\qquad
%   \subfigure[\scriptsize{$\text{DEO}$-SGD$\times$P16}]{\label{DEO_parallel}\includegraphics[width=2.2cm, height=2.2cm]{figures/NRPT_density_NRPT_iters_20000_chains_16_lr_0.01_0.5_sz_100_swap_rate_0.4_scale_2_window_1_seed_8.png}}\qquad
%   \subfigure[\scriptsize{$\text{DEO}_{\star}$-SGD$\times$P16}]{\label{deo_star_parallel}\includegraphics[width=2.3cm, height=2.2cm]{figures/NRPT_density_NRPT_iters_20000_chains_16_lr_0.01_0.5_sz_100_swap_rate_0.4_scale_2_window_8_seed_8.png}}
%     \vskip -0.05in
%   \caption{Simulations of the multi-modal distribution through different sampling algorithms. }
%   \label{multi_modal_simulation}
%   \vspace{-0.5em}
% \end{figure*}

==> chapters/checklist.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section*{Checklist}


% %%% BEGIN INSTRUCTIONS %%%
% The checklist follows the references.  Please
% read the checklist guidelines carefully for information on how to answer these
% questions.  For each question, change the default \answerTODO{} to \answerYes{},
% \answerNo{}, or \answerNA{}.  You are strongly encouraged to include a {\bf
% justification to your answer}, either by referencing the appropriate section of
% your paper or providing a brief inline description.  For example:
% \begin{itemize}
%   \item Did you include the license to the code and datasets? \answerYes{See Section~\ref{gen_inst}.}
%   \item Did you include the license to the code and datasets? \answerNo{The code and the data are proprietary.}
%   \item Did you include the license to the code and datasets? \answerNA{}
% \end{itemize}
% Please do not modify the questions and only use the provided macros for your
% answers.  Note that the Checklist section does not count towards the page
% limit.  In your paper, please delete this instructions block and only keep the
% Checklist section heading above along with the questions/answers below.
% %%% END INSTRUCTIONS %%%


\begin{enumerate}


\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{}
  \item Did you describe the limitations of your work?
    \answerYes{}
  \item Did you discuss any potential negative societal impacts of your work?
    \answerNA{}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{}
\end{enumerate}


\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerYes{}
        \item Did you include complete proofs of all theoretical results?
    \answerYes{}
\end{enumerate}


\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerYes{}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerYes{}
        \item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerYes{}
        \item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerNo{}
\end{enumerate}


\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
   \answerYes{}
  \item Did you mention the license of the assets?
   \answerNA{}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerNA{}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
     \answerNA{}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
     \answerNA{}
\end{enumerate}


\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerNA{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
   \answerNA{}
\end{enumerate}


\end{enumerate}
